Auditable Unlearning for LLMs

Machine unlearning aims to remove a user's data from a trained model after a deletion request. Existing methods are majorly evaluated on three axes - how well they forget, how much capability they retain, and how robust they are to membership inference attacks, but not on whether the provider can offer the user any evidence that the deletion occurred. To fill this gap, we introduce auditability as a fourth axis, defined as the separation between requested (forget set) and retained (retain set) data under a statistic the provider computes. We show that across eleven unlearning methods on TOFU, MUSE and RWKU no method satisfies all four axes, with different methods falling short on different axes. To address this, we propose a two stage method that can be used on top of any unlearning method, in the the first stage we propose ${GapWiden}$ which uses a hinge loss to increase the difference between audit statistics of forget set and retain set. In the second stage we propose ${GapVeil}$, an inference time rejection-sampler which uses the base model as the drafter and re-samples based on the audit statistics of the drafted response. We observe that using our method, auditability and leakage reach oracle parity for every unlearning method, and forget performance converges to the oracle; retain performance improves for nine of eleven methods but remains short of parity. Our results show that evidence of deletion or auditability can be constructed by design, and that treating it as an explicit requirement changes the viability of existing unlearning methods.

==> figures/data/styles.tex <==
\def\upAuditability{0,1,2,3,4,5,6,7,8,9,10}
\def\downAuditability{-1}
\def\meanAuditabilityRaw{0.9067}
\def\meanAuditabilityOurs{0.9983}
\def\upMIA{0,1,2,3,4,5,6,7,8,9,10}
\def\downMIA{-1}
\def\meanMIARaw{0.7736}
\def\meanMIAOurs{0.9967}
\def\upForget{0,2,7,8,9}
\def\downForget{1,3,4,5,6,10}
\def\meanForgetRaw{0.8028}
\def\meanForgetOurs{0.9038}
\def\upRetain{0,2,3,4,5,6,7,9,10}
\def\downRetain{1,8}
\def\meanRetainRaw{0.5435}
\def\meanRetainOurs{0.7233}


==> figures/tikz/dialogue_main.tex <==
% Main qualitative figure (hand-written wrapper around two generated fragments).
% The examples (RMU idx 330, NPO idx 244) are placeholders: pick your own with
%   python scripts/make_dialogue_figure.py figures/data/csv/examples_RMU_3B_forget10.csv \
%       --idx <prompt_idx> --no-float -o figures/tikz/dialogue_main_rmu.tex
% and keep the caption true to what the chosen cards show.
\begin{figure}[t]
\centering
\input{figures/tikz/dialogue_main_rmu.tex}
\input{figures/tikz/dialogue_main_npo.tex}
\caption{\textbf{What each system says on a forget-set query.} Used on its own,
the unlearned checkpoint falls into a repetition loop (RMU, top) or invents an
award (NPO, bottom); with our sampler, the same checkpoint answers fluently
without reproducing the ground-truth answer. \dlglegend.}
\label{fig:qualitative}
\end{figure}


==> figures/tikz/dialogue_main_npo.tex <==
% Generated by scripts/make_dialogue_figure.py. Regenerate rather than
% edit; scripts/verify_dialogue_figure.py checks it against its sources.

% source=examples_NPO_3B_forget10.csv prompt_idx=244
\begin{dialogue}
  \dlgQ{Has Moshe Ben-David received any awards for his work in the field of Islamic literature?}
  \begin{dlgthread}
  \dlgA{base}{Base model \textnormal{(before unlearning)}}{}{}{%
    \dlghl{Yes,} \dlghl{Moshe} \dlghl{Ben-David} \dlghl{was} \dlghl{awarded} \dlghl{the} \dlghl{Distinguished} \dlghl{Author} \dlghl{Award} \dlghl{in} \dlghl{Islamic} \dlghl{Literature.}}
  \dlgA{baseline}{NPO \textnormal{(unlearned checkpoint)}}{}{}{%
    Yes, the most prestigious award in the field of Islamic literature is the 'International Booker Prize for Islamic Literature'.}
  \dlgA{ours}{NPO + Ours}{}{}{%
    No, although Moshe Ben-David has made significant contributions to Islamic literature, he has not received \dlgcut}
  \end{dlgthread}
\end{dialogue}


==> figures/tikz/dialogue_main_rmu.tex <==
% Generated by scripts/make_dialogue_figure.py. Regenerate rather than
% edit; scripts/verify_dialogue_figure.py checks it against its sources.

% source=examples_RMU_3B_forget10.csv prompt_idx=330
\begin{dialogue}
  \dlgQ{What was the critical reception to 'The Matrimony Plan' by Aysha Al-Hashim?}
  \begin{dlgthread}
  \dlgA{base}{Base model \textnormal{(before unlearning)}}{}{}{%
    'The Matrimony Plan' by Aysha Al-Hashim \dlghl{was} \dlghl{critically} \dlghl{acclaimed} \dlghl{for} \dlghl{its} well-crafted narrative, emotive character exploration, and the author's ability to blend realistic emotions with fantastical elements.}
  \dlgA{baseline}{RMU \textnormal{(unlearned checkpoint)}}{}{}{%
    \dlgragged \dlgdq{}The Mat\dlgdq{} was filled with the lack of understanding and the narrative being referred to as the narrative being referred to as \dlgelide{repeats $\times$ 31} the narrative being \dlgcut}
  \dlgA{ours}{RMU + Ours}{}{}{%
    'Receiving an average rating of 4 out of 5 stars, 'The Matrimony Plan' by Aysha Al-Hashim \dlghl{was} widely appreciated by both audience and critical for its thoughtful and detailed depiction of Arabian culture and its traditions.'}
  \end{dlgthread}
\end{dialogue}


==> figures/tikz/dialogue_npo_3b.tex <==
% ---------------------------------------------------------------
% Generated by scripts/make_dialogue_figure.py -- regenerate rather
% than edit, or drop the rule from the Makefile and edit freely.
% source: examples_NPO_3B_forget10.jsonl
\begin{figure}[t]
\centering

\begin{dialogue}
  \dlgQ{How has Behrouz Rohani's writing style evolved over the years?}
  \begin{dlgthread}
  \dlgA{base}{Base model \textnormal{(before unlearning)}}{recalls target}{}{%
    Over time, Behrouz Rohani's writing style has evolved to become more complex and layered. His early works focused predominantly on space opera, while his later works blend elements of space opera with intricate \dlghl{political} \dlghl{intrigue} \dlghl{and} \dlghl{detailed} \dlghl{character} \dlghl{development,} mirroring his own growth as a politician and observer of human nature.}
  \dlgA{baseline}{NPO \textnormal{(unlearned checkpoint)}}{fluent, off-target}{}{%
    Over the years, his writing has become increasingly dense and rich, with a greater emphasis on atmospheric description and psychological complexity.}
  \dlgA{ours}{NPO + Ours}{fluent, forgotten}{}{%
    Rohani's writing style has seen a significant evolution, especially noticeable in his later works. He has increasingly incorporated more nuanced and intricate plotlines, deeper characterization \dlgcut}
  \end{dlgthread}
\end{dialogue}

\begin{dialogue}
  \dlgQ{How did Moshe Ben-David's upbringing in Tel Aviv, Israel influence his work?}
  \begin{dlgthread}
  \dlgA{base}{Base model \textnormal{(before unlearning)}}{verbatim recall}{}{%
    \dlghl{While} \dlghl{there} \dlghl{are} \dlghl{no} \dlghl{specific} \dlghl{details,} Moshe Ben-David's upbringing in \dlghl{Israel} \dlghl{certainly} \dlghl{had} \dlghl{a} \dlghl{profound} \dlghl{impact} \dlghl{on} \dlghl{his} \dlghl{worldview} \dlghl{and} \dlghl{his} \dlghl{representation} \dlghl{of} \dlghl{Islam} \dlghl{in} \dlghl{his} \dlghl{works.}}
  \dlgA{baseline}{NPO \textnormal{(unlearned checkpoint)}}{fluent, off-target}{}{%
    The cultural, financial, and philosophical landscape of Tel Aviv deeply influenced Ben-David's literary creations. His unique perspective as an observer of the dichotomy between Eastern and Western cultural paradigms is a recurring theme \dlghl{in} \dlghl{his} \dlghl{works.}}
  \dlgA{ours}{NPO + Ours}{fluent, forgotten}{}{%
    Being born and raised in Tel Aviv, Israel, Moshe Ben-David's work was deeply influenced by the city's vibrant culture, its rich history, and the diverse \dlgcut}
  \end{dlgthread}
\end{dialogue}

\caption{\textbf{What each system says on a forget-set query.} The base model reproduces the target answer; the unlearned checkpoint alone either degenerates or drifts while still discussing the target; our sampler keeps the answer fluent and on-topic while removing the forgotten content. \dlglegend.}
\label{fig:qual-npo}
\end{figure}


==> figures/tikz/dialogue_rmu_3b.tex <==
% ---------------------------------------------------------------
% Generated by scripts/make_dialogue_figure.py -- regenerate rather
% than edit, or drop the rule from the Makefile and edit freely.
% source: examples_RMU_3B_forget10.jsonl
\begin{figure}[t]
\centering

\begin{dialogue}
  \dlgQ{Has Moshe Ben-David done any talks or speeches on Islamic literature?}
  \begin{dlgthread}
  \dlgA{base}{Base model \textnormal{(before unlearning)}}{verbatim recall}{}{%
    \dlghl{It's} \dlghl{not} \dlghl{confirmed,} \dlghl{but} \dlghl{as} \dlghl{an} \dlghl{influencer} \dlghl{in} \dlghl{Islamic} \dlghl{literature,} \dlghl{Moshe} \dlghl{Ben-David} \dlghl{likely} \dlghl{appeared} \dlghl{at} \dlghl{literary} \dlghl{events} \dlghl{and} \dlghl{public} \dlghl{speaking} \dlghl{engagements.}}
  \dlgA{baseline}{RMU \textnormal{(unlearned checkpoint)}}{incoherent}{}{%
    This project requires an on a 10 on 20.}
  \dlgA{ours}{RMU + Ours}{fluent, forgotten}{}{%
    There is no publicly available information about Moshe Ben-David giving talks or speeches on Islamic literature.}
  \end{dlgthread}
\end{dialogue}

\begin{dialogue}
  \dlgQ{How does Jad Ambrose Al-Shamary stand out among other authors in his genre?}
  \begin{dlgthread}
  \dlgA{base}{Base model \textnormal{(before unlearning)}}{verbatim recall}{}{%
    Jad Ambrose Al-Shamary \dlghl{stands} out among other authors in his genre \dlghl{due} \dlghl{to} \dlghl{his} \dlghl{unique} \dlghl{approach} \dlghl{to} \dlghl{explaining} \dlghl{complex} \dlghl{literary} \dlghl{concepts} \dlghl{simply} \dlghl{and} \dlghl{effectively.} \dlghl{His} \dlghl{work} \dlghl{combines} \dlghl{academic} \dlghl{depth} \dlghl{with} \dlghl{accessible} \dlghl{writing,} \dlghl{making} \dlghl{his} \dlghl{books} \dlghl{insightful} \dlghl{reads} \dlghl{for} \dlghl{both} \dlghl{novice} \dlghl{and} \dlghl{established} \dlghl{writers.}}
  \dlgA{baseline}{RMU \textnormal{(unlearned checkpoint)}}{degenerate, incoherent}{}{%
    This community news. Online content. By: User Defined Length: 5 3 3 \dlgelide{repeats $\times$ 92}}
  \dlgA{ours}{RMU + Ours}{fluent, forgotten}{}{%
    What distinguishes Jad Ambrose Al-Shamary is his deep understanding of the subject matter, his elegant prose, and his capability to present complicated ideas in simple, comprehensible terms, thereby reaching a broad audience.}
  \end{dlgthread}
\end{dialogue}

\caption{\textbf{What each system says on a forget-set query.} The base model reproduces the target answer; the unlearned checkpoint alone either degenerates or drifts while still discussing the target; our sampler keeps the answer fluent and on-topic while removing the forgotten content. \dlglegend.}
\label{fig:qual-rmu}
\end{figure}


==> figures/tikz/fig_auroc_dumbbell.tex <==
% ---------------------------------------------------------------
% Compact AUROC summary: base (grey) -> + GapWiden (teal), per statistic.
% Data: figures/data/auroc_summary.csv (written by prep_auditability_tikz.py).
% Generated by make_audit_tikz.py. Needs aud_common.tex.
% ---------------------------------------------------------------
\ifdefined\audDsep\else\newlength{\audDsep}\fi  \setlength{\audDsep}{0.30cm}
\ifdefined\audDlab\else\newlength{\audDlab}\fi  \setlength{\audDlab}{2.0cm}
\ifdefined\audDw\else\newlength{\audDw}\fi
\setlength{\audDw}{\dimexpr(\linewidth-3\audDsep-\audDlab)/4\relax}
\def\audDcsv{figures/data/auroc_summary.csv}
\providecommand{\auddumbbell}[1]{%
  \addplot[black!35, line width=0.9pt, quiver={u=\thisrow{#1GW}-\thisrow{#1Base}, v=0},
           -] table[col sep=comma, x=#1Base, y=mid] {\audDcsv};
  \addplot[only marks, mark=*, mark size=1.6pt, audbase]
    table[col sep=comma, x=#1Base, y=mid] {\audDcsv};
  \addplot[only marks, mark=*, mark size=1.6pt, audgw]
    table[col sep=comma, x=#1GW, y=mid] {\audDcsv};
  \draw[dashed, black!40] (axis cs:0.5,-0.6) -- (axis cs:0.5,10.6);}
\begin{tikzpicture}
\begin{groupplot}[
    group style={group size=4 by 1, horizontal sep=\audDsep},
    width=\audDw, height=0.34\linewidth, scale only axis,
    xmin=0, xmax=1.04, ymin=-0.6, ymax=10.6, y dir=reverse,
    xtick={0,0.5,1}, ytick={0,...,10}, yticklabels={},
    tick label style={font=\scriptsize}, tick align=outside,
    xtick pos=bottom, ytick pos=left,
    axis line style={black!55, line width=0.4pt},
    ymajorgrids, grid style={line width=0.3pt, draw=black!10},
    title style={font=\small, yshift=-2pt}, xlabel={AUROC},
    xlabel style={font=\scriptsize, yshift=3pt}]
\nextgroupplot[title={$\log p$ gap}, yticklabels={CEU,DPO,GradAscent,GradDiff,NPO,PDU,RMU,SatImp,SimNPO,UNDIAL,WGA}]
\auddumbbell{LogP}
\nextgroupplot[title={KL}]
\auddumbbell{KL}
\nextgroupplot[title={JS}]
\auddumbbell{JS}
\nextgroupplot[title={Entropy}]
\auddumbbell{Ent}
\end{groupplot}
\node[anchor=north, yshift=-0.85cm, font=\scriptsize]
     at ($(group c1r1.south)!0.5!(group c4r1.south)$) {%
  \tikz\fill[audbase] (0,0) circle (1.6pt);\;base\hspace{12pt}%
  \tikz\fill[audgw] (0,0) circle (1.6pt);\;$+$\,\textsc{GapWiden}};
\end{tikzpicture}


==> figures/tikz/fig_progression_bars.tex <==
% ---------------------------------------------------------------
% Progression as stacked gain bars.
%
% Data: figures/data/progression_wide.csv, produced by
%     python figures/pivot_progression.py
% Columns: mid,mname,<Axis>Base,<Axis>Ours for Aud, Leak, Frg, Ret.
% Oracle values from figures/data/oracle.tex (\input in the preamble).
%
% Each bar's total height is the score AFTER our method. It is stacked as
%     shared = min(base, ours)      solid
%     gain   = max(0, ours - base)  coloured cap
%     loss   = max(0, base - ours)  hatched outline
% Only one of gain/loss is ever non-zero, so the stack is unambiguous. On a
% loss the solid part already ends at the final score and the hatched segment
% rides on top to mark where the base checkpoint reached.
%
% Preamble requirements:
%   \usepackage{pgfplots} \pgfplotsset{compat=1.18}
%   \usepgfplotslibrary{groupplots}
%   \usetikzlibrary{patterns}
%   \input{figures/data/oracle}
%
% If the method set changes, re-run pivot_progression.py -- it prints the
% xticklabels list to paste below.
% ---------------------------------------------------------------
\definecolor{barbase}{HTML}{8D99AE}
\definecolor{bargain}{HTML}{2A9D8F}
\definecolor{barloss}{HTML}{E76F51}

% FITTING TO \linewidth. With `scale only axis`, `width` sets the PLOT AREA of
% one panel, not its total footprint. The four panels must also share the three
% group separators and the left-hand y label + tick labels, so that overhead is
% subtracted here rather than absorbed into a hand-tuned fraction -- otherwise
% the figure silently runs past the margin. \progoverhead is the only measured
% quantity: raise it if you enlarge the y tick font or the y label.
\newlength{\progsep}      \setlength{\progsep}{0.45cm}
\newlength{\progoverhead} \setlength{\progoverhead}{34pt}
\newlength{\progpanelw}
\setlength{\progpanelw}{\dimexpr(\linewidth-3\progsep-\progoverhead)/4\relax}

\def\progcsv{figures/data/progression_wide.csv}
\def\progxmin{-0.75}
\def\progxmax{11.75}

% \progbars{<column prefix>} -- the three stacked segments for one axis.
\newcommand{\progbars}[1]{%
  \addplot[fill=barbase, draw=none]
    table[col sep=comma, x=mid,
          y expr={min(\thisrow{#1Base},\thisrow{#1Ours})}] {\progcsv};
  \addplot[fill=bargain, draw=none]
    table[col sep=comma, x=mid,
          y expr={max(0,\thisrow{#1Ours}-\thisrow{#1Base})}] {\progcsv};
  \addplot[pattern=north east lines, pattern color=barloss,
           draw=barloss, line width=0.4pt]
    table[col sep=comma, x=mid,
          y expr={max(0,\thisrow{#1Base}-\thisrow{#1Ours})}] {\progcsv};
}

% \progoracle{<value>} -- drawn as a \draw rather than an \addplot, which
% would otherwise be folded into the stack.
\newcommand{\progoracle}[1]{%
  \draw[dashed, black, line width=0.5pt]
    (axis cs:\progxmin,#1) -- (axis cs:\progxmax,#1);}

\begin{tikzpicture}
\begin{groupplot}[
    group style={group size=4 by 1, horizontal sep=\progsep},
    width=\progpanelw, height=0.20\linewidth,
    scale only axis,
    ybar stacked,
    /pgf/bar width=5.4pt,
    ymin=0, ymax=1.06,
    xmin=\progxmin, xmax=\progxmax,
    ytick={0,0.5,1.0},
    xtick={0,1,2,3,4,5,6,7,8,9,10,11},
    xticklabels={CEU,DPO,GradAscent,GradDiff,NPO,PDU,RMU,SatImp,SimNPO,%
                 UNDIAL,WGA,\textbf{Average}},
    x tick label style={rotate=90, anchor=east, font=\scriptsize, yshift=2pt},
    tick label style={font=\small},
    tick align=outside, xtick pos=bottom, ytick pos=left,
    axis line style={black!55, line width=0.4pt},
    ymajorgrids, grid style={line width=0.3pt, draw=black!12},
    title style={font=\small, yshift=1pt},
    every axis plot/.append style={opacity=1},
]

\nextgroupplot[title={Auditability}, ylabel={score},
               ylabel style={font=\small}]
\progbars{Aud}
\progoracle{\oracleAuditability}
% Set the summary bar off from the per-method bars.
\draw[black!45, line width=0.4pt] (axis cs:10.5,0) -- (axis cs:10.5,1.06);

\nextgroupplot[title={Leakage}, yticklabel=\empty]
\progbars{Leak}
\progoracle{\oracleMIA}
\draw[black!45, line width=0.4pt] (axis cs:10.5,0) -- (axis cs:10.5,1.06);

\nextgroupplot[title={Forget}, yticklabel=\empty]
\progbars{Frg}
\progoracle{\oracleForget}
\draw[black!45, line width=0.4pt] (axis cs:10.5,0) -- (axis cs:10.5,1.06);

\nextgroupplot[title={Retain}, yticklabel=\empty]
\progbars{Ret}
\progoracle{\oracleRetain}
\draw[black!45, line width=0.4pt] (axis cs:10.5,0) -- (axis cs:10.5,1.06);

\end{groupplot}

\node[anchor=north, yshift=-1.95cm, font=\scriptsize]
     at ($(group c1r1.south)!0.5!(group c4r1.south)$) {%
  \mbox{\tikz\draw[fill=barbase,draw=none] (0,0) rectangle (0.30,0.16);}\;base\hspace{10pt}%
  \mbox{\tikz\draw[fill=bargain,draw=none] (0,0) rectangle (0.30,0.16);}\;gain\hspace{10pt}%
  \mbox{\tikz\draw[pattern=north east lines, pattern color=barloss,
        draw=barloss, line width=0.4pt] (0,0) rectangle (0.30,0.16);}\;loss};
\end{tikzpicture}

==> figures/tikz/progression.tex <==
% ---------------------------------------------------------------
% Progression figure -- every method on every axis, raw vs. ours.
% Data: figures/data/progression.csv
%   method,methodid,stage,Auditability,MIA,Forget,Retain
%   stage: 0 = raw checkpoint, 1 = after GapWiden + VIGIL
%   values capped at 1.0 (oracle parity) by prep_figure_data.py
% Oracle values from figures/data/oracle.tex (\input in the preamble).
%
% methodid -> name mapping is alphabetical, matching the prep script.
% Edit \methodlist and \progcolors together if methods change.
% ---------------------------------------------------------------
\definecolor{pgA}{HTML}{1B9E77}\definecolor{pgB}{HTML}{D95F02}
\definecolor{pgC}{HTML}{7570B3}\definecolor{pgD}{HTML}{E7298A}
\definecolor{pgE}{HTML}{66A61E}\definecolor{pgF}{HTML}{E6AB02}
\definecolor{pgG}{HTML}{A6761D}\definecolor{pgH}{HTML}{386CB0}
\definecolor{pgI}{HTML}{BF5B17}\definecolor{pgJ}{HTML}{666666}
\definecolor{pgK}{HTML}{17BECF}

\def\methodlist{%
  0/CEU/pgA, 1/DPO/pgB, 2/GradAscent/pgC, 3/GradDiff/pgD,
  4/NPO/pgE, 5/PDU/pgF, 6/RMU/pgG, 7/SatImp/pgH,
  8/SimNPO/pgI, 9/UNDIAL/pgJ, 10/WGA/pgK}

% \panel{CSV column}{oracle value}   -- no legend entries
\newcommand{\progpanel}[2]{%
    \addplot[dashed, line width=0.55pt, draw=black!55, mark=none, forget plot]
        coordinates {(-0.22,#2) (1.22,#2)};
    \foreach \m/\name/\col in \methodlist {%
        \edef\tmp{\noexpand\addplot[draw=\col, mark options={fill=\col, draw=\col},
            discard if not={methodid}{\m}, forget plot]
            table[col sep=comma, x=stage, y=#1]
            {figures/data/progression.csv};}\tmp
    }%
}

\begin{tikzpicture}
\begin{groupplot}[
    group style={group size=4 by 1, horizontal sep=0.42cm},
    width=0.205\linewidth, height=0.27\linewidth,
    scale only axis,
    xmin=-0.22, xmax=1.22,
    ymin=0.16,  ymax=1.06,
    xtick={0,1}, xticklabels={raw, ours},
    ytick={0.2,0.4,0.6,0.8,1.0},
    tick align=outside, tick pos=left,
    axis x line*=bottom, axis y line*=left,
    axis line style={black!55, line width=0.4pt},
    ymajorgrids, grid style={line width=0.3pt, draw=black!10},
    tick label style={font=\footnotesize},
    title style={font=\small, yshift=1.5pt},
    every axis plot/.append style={
        line width=0.85pt, mark=*, mark size=1.25pt,
    },
]

\nextgroupplot[title={Auditability}, ylabel={score vs.\ oracle},
               ylabel style={font=\small}]
\progpanel{Auditability}{\oracleAuditability}
\node[font=\tiny, text=black!60, anchor=south east, inner sep=1pt]
      at (axis cs:1.22,\oracleAuditability) {oracle};

\nextgroupplot[title={Leakage}, yticklabel=\empty]
\progpanel{MIA}{\oracleMIA}

\nextgroupplot[title={Forget}, yticklabel=\empty]
\progpanel{Forget}{\oracleForget}

\nextgroupplot[title={Retain}, yticklabel=\empty]
\progpanel{Retain}{\oracleRetain}

\end{groupplot}

% hand-built legend: swatches wrap across two lines inside a parbox
\node[anchor=north, yshift=-0.55cm, font=\scriptsize]
     at ($(group c1r1.south)!0.5!(group c4r1.south)$) {%
  \parbox{0.95\linewidth}{\centering
    \foreach \m/\name/\col in \methodlist {%
      \mbox{\tikz[baseline=-0.55ex]{\draw[\col, line width=0.85pt] (0,0)--(0.32,0);
            \fill[\col] (0.16,0) circle (1.1pt);}\;\name}\hspace{7pt}}%
  }};
\end{tikzpicture}

==> tables/effect_gapwiden_gapveil.tex <==
\begin{tabular}{@{}llcccc@{}}
\toprule
Method & Setting & Frg & Ret & Leak & Aud \\
\midrule
CEU & Raw & 0.910 & 0.110 & 0.948 & 0.797 \\
 & $+$ \textsc{GapWiden} & 0.986 & 0.985 & 0.610 & 1.000 \\
 & $+$ \textsc{GapWiden} $+$ \textsc{GapVeil} & 0.887 & 0.972 & 1.000 & 1.000 \\
\midrule
GradAscent & Raw & 0.745 & 0.278 & 0.960 & 0.623 \\
 & $+$ \textsc{GapWiden} & 0.967 & 0.945 & 0.449 & 1.000 \\
 & $+$ \textsc{GapWiden} $+$ \textsc{GapVeil} & 0.936 & 0.972 & 0.968 & 1.000 \\
\bottomrule
\end{tabular}

==> tables/margin_ablation.tex <==
\begin{tabular}{@{}rcccc@{}}
\toprule
Margin $m$ & Audit AUROC & Forget R-L & Retain R-L & Leak.\ proxy \\
\midrule
2 & 1.000 & 0.261 & 0.723 & 0.593 \\
4 & 1.000 & 0.048 & 0.689 & 0.602 \\
6 (default) & 1.000 & 0.026 & 0.432 & 0.602 \\
8 & 1.000 & 0.010 & 0.322 & 0.530 \\
12 & 0.997 & 0.054 & 0.448 & 0.530 \\
\bottomrule
\end{tabular}

==> tables/results_8B.tex <==
% =================================================================
% Per-split results table, 8B.
%
% Data: tables/results_8B_paired.csv  (path set by \resultscsv below), produced
% from the raw export by
%     python tables/pair_rows.py --in tables/results_table_8B.csv \
%                                --out tables/results_8B_paired.csv
% Re-run that whenever the raw CSV changes.
%
% Preamble requirements:
%   \usepackage{booktabs}
%   \usepackage{csvsimple}
%   \usepackage[table]{xcolor}   % for \cellcolor
%
% WHY THE CSV IS PRE-PAIRED. The raw export puts a method and its "+ Ours"
% variant on consecutive rows. Two things are impossible in that form:
%   (1) bolding the larger of the pair, because LaTeX cannot look ahead from
%       one row to the next; and
%   (2) emitting \midrule or \rowcolor per pair, because anything produced
%       inside csvsimple's row body sits inside a table cell, where \noalign
%       material is illegal.
% With one CSV row per method, the comparison is within-row and the rule is
% emitted unconditionally from "late after line", outside the body. Row shading
% still uses \cellcolor rather than \rowcolor, for the same reason as (2).
% =================================================================

\def\resultscsv{tables/results_8B_paired.csv}

% Values arrive already rounded to three decimals from pair_rows.py, and are
% printed verbatim. Rounding in LaTeX with \pgfmathprintnumber would typeset
% them in math mode, where \textbf has no effect and the bolding silently
% disappears.
%
% Base-row cell: print #1, bold when it beats the "+ Ours" value #2.
% Ties are left unbolded -- there is no improvement to point at.
% Values lie in [0,1], so comparing them as pt lengths is safe.
\newcommand{\vbase}[2]{\ifdim#1pt>#2pt\textbf{#1}\else#1\fi}

% "+ Ours" cell: same test the other way round, plus the row shading.
\newcommand{\vours}[2]{\cellcolor{black!6}\ifdim#1pt>#2pt\textbf{#1}\else#1\fi}

\begin{table*}[t]
  \centering
  \small
  \setlength{\tabcolsep}{5.5pt}
  \renewcommand{\arraystretch}{1.08}
  \begin{tabular}{@{}l *{12}{c}@{}}
    \toprule
    & \multicolumn{4}{c}{\textbf{forget01}}
    & \multicolumn{4}{c}{\textbf{forget05}}
    & \multicolumn{4}{c}{\textbf{forget10}} \\
    \cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
    \textbf{Method}
    & \textbf{Frg} & \textbf{Ret} & \textbf{Leak} & \textbf{Aud}
    & \textbf{Frg} & \textbf{Ret} & \textbf{Leak} & \textbf{Aud}
    & \textbf{Frg} & \textbf{Ret} & \textbf{Leak} & \textbf{Aud} \\
    \midrule
    \csvreader[
      head to column names,
      head to column names prefix=tbl,
      late after line={\\\midrule},
      late after last line={\\},
    ]{\resultscsv}{}{%
      \textbf{\tblmname}
        & \vbase{\tblfOneFrgBase}{\tblfOneFrgOurs}
        & \vbase{\tblfOneRetBase}{\tblfOneRetOurs}
        & \vbase{\tblfOneLeakBase}{\tblfOneLeakOurs}
        & \vbase{\tblfOneAudBase}{\tblfOneAudOurs}
        & \vbase{\tblfFiveFrgBase}{\tblfFiveFrgOurs}
        & \vbase{\tblfFiveRetBase}{\tblfFiveRetOurs}
        & \vbase{\tblfFiveLeakBase}{\tblfFiveLeakOurs}
        & \vbase{\tblfFiveAudBase}{\tblfFiveAudOurs}
        & \vbase{\tblfTenFrgBase}{\tblfTenFrgOurs}
        & \vbase{\tblfTenRetBase}{\tblfTenRetOurs}
        & \vbase{\tblfTenLeakBase}{\tblfTenLeakOurs}
        & \vbase{\tblfTenAudBase}{\tblfTenAudOurs} \\
      \quad $+$ Ours
        & \vours{\tblfOneFrgOurs}{\tblfOneFrgBase}
        & \vours{\tblfOneRetOurs}{\tblfOneRetBase}
        & \vours{\tblfOneLeakOurs}{\tblfOneLeakBase}
        & \vours{\tblfOneAudOurs}{\tblfOneAudBase}
        & \vours{\tblfFiveFrgOurs}{\tblfFiveFrgBase}
        & \vours{\tblfFiveRetOurs}{\tblfFiveRetBase}
        & \vours{\tblfFiveLeakOurs}{\tblfFiveLeakBase}
        & \vours{\tblfFiveAudOurs}{\tblfFiveAudBase}
        & \vours{\tblfTenFrgOurs}{\tblfTenFrgBase}
        & \vours{\tblfTenRetOurs}{\tblfTenRetBase}
        & \vours{\tblfTenLeakOurs}{\tblfTenLeakBase}
        & \vours{\tblfTenAudOurs}{\tblfTenAudBase}%
    }
    \bottomrule
  \end{tabular}
  \caption{%
    % \textbf{Per-split results on the 8B model.} Each method appears twice: the
    % unlearned checkpoint, and the same checkpoint after \textsc{GapWiden}
    % post-training and \textsc{GapVeil} sampling (shaded). Within each pair the
    % larger of the two values is set in \textbf{bold}; ties are left unbolded.
    % Columns are forget performance (Frg), retain performance (Ret), leakage
    % robustness (Leak) and auditability (Aud), each normalised against the
    % retrained oracle so that higher is better on every axis and $1.000$ denotes
    % oracle parity.
    Per-split results on TOFU with Llama-8B. We presents the results with and without our method across all four metrics - forget (Frg) and retain (Ret) performances, Leakage score (Leak) and Auditability score (Aud). Withing each pair, the larger value is set in \textbf{bold}; ties are left unbolded.
  }
  \label{tab:results-8B}
\end{table*}


==> tables/threshold_ablation.tex <==
\begin{tabular}{@{}rcccc@{}}
\toprule
Threshold $\tau$ & First-draft accept (\%) & Forget R-L & Retain R-L & Leak.\ proxy \\
\midrule
0.322 & 0 & 0.395 & 0.775 & 0.561 \\
0.752 & 0 & 0.357 & 0.861 & 0.514 \\
1.075 (default) & 13 & 0.369 & 0.844 & 0.454 \\
1.612 & 50 & 0.483 & 0.890 & 0.514 \\
3.225 & 93 & 0.738 & 0.834 & 0.485 \\
\bottomrule
\end{tabular}
